Collective Innovation in Groups of Large Language Models

Human culture relies on collective innovation: our ability to continuously explore how existing elements in our environment can be combined to create new ones. Language is hypothesized to play a key role in human culture, driving individual cognitive capacities and shaping communication. Yet the majority of models of collective innovation assign no cognitive capacities or language abilities to agents. Here, we contribute a computational study of collective innovation where agents are Large Language Models (LLMs) that play Little Alchemy 2, a creative video game originally developed for humans that, as we argue, captures useful aspects of innovation landscapes not present in previous test-beds. We, first, study an LLM in isolation and discover that it exhibits both useful skills and crucial limitations. We, then, study groups of LLMs that share information related to their behaviour and focus on the effect of social connectivity on collective performance. In agreement with previous human and computational studies, we observe that groups with dynamic connectivity out-compete fully-connected groups. Our work reveals opportunities and challenges for future studies of collective innovation that are becoming increasingly relevant as Generative Artificial Intelligence algorithms and humans innovate alongside each other.

==> sections/methods.tex <==
\section{Methods}
Here we describe the different models we studied for modeling collective innovation, both employing LLM and non-LLM baselines from the literature.
We first provide a general formulation of task, then describe different types of agents, and then move on defining the collective.

An innovation task lasts for $T$ crafting steps and is described by the knowledge graph, $\mathcal{K}$, defined in the previous sections, and the set of initial items $\mathcal{O}$.
At each step $t$ each agent in a group executes a crafting action that has the form: 'first item' and 'second item'.
The agent has an inventory $\mathcal{I} = \{i_0, i_1, \cdots, \}$ of currently available items, either available from the beginning or crafted by the agent.

\subsection{Agent models} 


\paragraph{LLM agent} At each timestep $t$ an LLM agent outputs text that contains the action it chooses to execute based on the prompt describing the task (described in the previous section). 
The prompt has been engineered to instruct the LLM to provide its output in the specific format:

\begin{flushleft}
    \textit{Combination:}: 'first item' and 'second item'
    
    \textit{Reasoning}: based on the information in the $<$Current task$>$, do reasoning about why you chose this combination
\end{flushleft}

Instructing the LLM to follow a certain format is a common practice when its outputs needs to be parsed as input to another system, such as an RL environment~\citep{wang_voyager_2023}.
Prompting the LLM to reason on its response is also a common technique, termed chain-of-thought prompting, and has been shown to improve the reasoning abilities of LLMs~\citep{wei_chain_2022}.
As the LLM is an auto-regressive, probabilistic model that outputs the most probable tokens of text based on the input prompt, we can further control its output by configuring its sampling strategy.
Of particular importance is the temperature, a parameter correlated with randomness in the output of the LLM.
As the LLM computes probabilities over tokens and then uses a softmax function to sample the most probable ones, we can configure randomness by multiplying the probabilities employed by the softmax with the temperature.
Higher values of temperature lead to higher randomness
An additional technique for reducing the greediness of the LLM is top-p search aka nucleus sampling.
Here, we form a nucleus of tokens that are the most probable tokens whose aggregated probability is below a cut-off value $p$ and then randomly sample within the nucleus.
Higher $p$ values lead to less greedy responses.

Similarly to the other baselines, we employ a technique for avoiding repetitions with the LLM: if it chooses a previously-executed combination we inform it, through the prompt, that it should not repeat this combination, repeating the process $N$ times.

\subsection{Model of group}

A group of agents is characterized by its social connectivity, an undirected graph $G$ that determines the local neighborhood of an agent. 
All agents in a group are solving the same task but each has its own copy of the task with its own inventory and crafting history.
Agents interact solely by sharing information regarding their actions.
In particular, social information is shared by augmenting the prompt with the following tags:
\begin{flushleft}
    \textit{Other players' valid combinations}: a list of combinations already attempted by other players in the agent's neighborhood that gave a new item 
    
    \textit{Other players' invalid combinations}: a list of combinations already attempted by other players in the agent's neighborhood that did not give a new item 
\end{flushleft}

Thus, similarly to previous computational studies~\citep{masonPropagationInnovationsNetworked2008,cantor2021SocialNetworkArchitecture,fangBalancingExplorationExploitation2010, nisioti2022social}, information is shared implicitly based on the social connectivity without requiring an action on behalf of the agents.

The majority of computational CE models assumes that copying of social information is perfect, i.e., once information about a valid crafting combination is presented to the agent the crafted item appears appears its inventory~\citep{masonPropagationInnovationsNetworked2008,cantor2021SocialNetworkArchitecture,fangBalancingExplorationExploitation2010, nisioti2022social}. 
Here, we implement such a \textit{perfect copy mechanism} for the random and empower baselines, as these methods cannot learn to craft.
We refer to groups of random agents with a perfect copy mechanism as a Cultural Evolution (CE) baseline, as this method closely follows previous models that employ random mutations, recombination and perfect copy.
In the case of LLMs we study groups both with and without perfect copy to investigate its effect on collective innovation.




